Taylor States in Stellarators: A Fast High-order Boundary Integral Solver

We present a boundary integral equation solver for computing Taylor relaxed states in non-axisymmetric solid and shell-like toroidal geometries. The computation of Taylor states in these geometries is a key element for the calculation of stepped pressure stellarator equilibria. The integral representation of the magnetic field in this work is based on the generalized Debye source formulation, and results in a well-conditioned second-kind boundary integral equation. The integral equation solver is based on a spectral discretization of the geometry and unknowns, and the computation of the associated weakly-singular integrals is performed with high-order quadrature based on a partition of unity. The resulting scheme for applying the integral operator is then coupled with an iterative solver and suitable preconditioners. Several numerical examples are provided to demonstrate the accuracy and efficiency of our method, and a direct comparison with the leading code in the field is reported.

==> makefile <==
###
## generic makefile for latex projects
## Author: Abtin Rahimian
###

###
## Plain 'make' should work most of the time, other useful patterns are
##  $ make help              #to see this
##  $ make verb              #for debugging
##  $ make nobib             #for faster compilation
##  $ make PROJ=name         #for project with different name from the dir
##  $ make OUTEXT=dvi        #for dvi output with latex compiler
##
## to have a faster compilation, this does most of passes in quiet
## mode. The downside is that it hides the error in case of
## failure. To see the error either "make verb" or "make VERB='yes'".
###

## user options
VERB	= yes
NOBIB   = no
PROJ    = main #$(notdir $(shell pwd))#defaults to dirname
LXX     = ${PDFLATEX}
OUTEXT  = pdf
SUMMARY = grep "\(error\|warn\|warning\|repeated\|skipping\)" -in --color
SYNC    = -synctex=1
ONEPASS = no
FIGRES  = 300

## programs
PDFLATEX = pdflatex
LATEX	 = latex
BIB	 = bibtex
DVI	 = dvipdf
PS	 = ps2pdf

## internal flag
QUIET	 =
LXFLAG 	 = -file-line-error -halt-on-error -shell-escape ${SYNC}
LXDFLAG  = ${LXFLAG}
BIBEXT   = bbl
INTEXT   = out

ifeq (${VERB},no)
  QUIET = -interaction=batchmode
endif

ifeq (${NOBIB},yes)
  BIBEXT = nobbl
endif

ifeq (${ONEPASS},no)
  LXFDFLAG += -draftmode
else
  INTEXT    = ${BIBEXT}
endif

TEXFILES = $(shell ls *.tex *.bib)

## project rules ##########################################################
###########################################################################
all: $(addsuffix .${OUTEXT}, ${PROJ})

## utility rules ##########################################################
###########################################################################
bib: $(addsuffix .${BIBEXT}, ${PROJ})

help:
	@head -18 ${MAKEFILE_LIST}

verb:   ## verbose make
	${MAKE} VERB=yes all

nobib:
	${MAKE} NOBIB=yes all

compress:
	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4    	\
	-dPDFSETTINGS=/printer -dNOPAUSE -dQUIET -dBATCH   	\
	-dDownsampleColorImages=true			 	\
	-dDownsampleGrayImages=true 				\
	-dDownsampleMonoImages=true 				\
        -dColorImageResolution=${FIGRES}			\
        -dGrayImageResolution=${FIGRES}				\
        -dMonoImageResolution=${FIGRES}				\
	-dColorImageDownsampleThreshold=1.5 			\
	-dGrayImageDownsampleThreshold=1.5 			\
	-dMonoImageDownsampleThreshold=1.5 			\
	-sOutputFile=${PROJ}-cmprs.pdf ${PROJ}.pdf

## generic rules ##########################################################
###########################################################################
%.pdf:${TEXFILES}
	${MAKE} LXX=${PDFLATEX} $*.${INTEXT}

%.dvi:${TEXFILES}
	${MAKE} LXX=${LATEX} $*.${INTEXT}

%.out:%.tex ${TEXFILES} %.${BIBEXT}
	${LXX} ${QUIET} ${LXDFLAG} $<
	${LXX} ${QUIET} ${LXFLAG} $<
	${SUMMARY} $*.log $*.blg
#	${MAKE} clean

%.aux:%.tex ${TEXFILES}
	${LXX} ${QUIET} ${LXDFLAG} $<

%.${BIBEXT}:%.aux
	-${BIB} $* 1>/dev/null
	-${SUMMARY} $*.blg

%.nobbl:%.aux
	@echo "skipping the bib make step"

clean:
	${RM} *out *-blx.bib *run.xml *.nav *.snm *.toc *.cb *.cb2 *.spl *.cpt *.tdo *.lof *.lot *.auxlock figs/*.log figs/*.spl *.upa

cleaner:
	${MAKE} clean
	${RM} *log *blg $(addsuffix .aux, ${PROJ}) $(addsuffix .synctex.gz, ${PROJ})
	${RM} figs/*.dpth figs/*.md5 figs/*.dep
cleanest:
	${MAKE} cleaner
	${RM} $(addsuffix .pdf, ${PROJ}) $(addsuffix .dvi, ${PROJ}) $(addsuffix .${OUTEXT}, ${PROJ}) $(addsuffix .bbl, ${PROJ}) figs/tikz-external-* figs/${PROJ}-*

.PHONY: clean cleaner cleanest
.SUFFIXES:
.SECONDARY:

